G3Reg: Pyramid Graph-based Global Registration using Gaussian Ellipsoid Model

This study introduces a novel framework, G3Reg, for fast and robust global registration of LiDAR point clouds. In contrast to conventional complex keypoints and descriptors, we extract fundamental geometric primitives, including planes, clusters, and lines (PCL) from the raw point cloud to obtain low-level semantic segments. Each segment is represented as a unified Gaussian Ellipsoid Model (GEM), using a probability ellipsoid to ensure the ground truth centers are encompassed with a certain degree of probability. Utilizing these GEMs, we present a distrust-and-verify scheme based on a Pyramid Compatibility Graph for Global Registration (PAGOR). Specifically, we establish an upper bound, which can be traversed based on the confidence level for compatibility testing to construct the pyramid graph. Then, we solve multiple maximum cliques (MAC) for each level of the pyramid graph, thus generating the corresponding transformation candidates. In the verification phase, we adopt a precise and efficient metric for point cloud alignment quality, founded on geometric primitives, to identify the optimal candidate. The algorithm's performance is validated on three publicly available datasets and a self-collected multi-session dataset. Parameter settings remained unchanged during the experiment evaluations. The results exhibit superior robustness and real-time performance of the G3Reg framework compared to state-of-the-art methods. Furthermore, we demonstrate the potential for integrating individual GEM and PAGOR components into other registration frameworks to enhance their efficacy. Code: https://github.com/HKUST-Aerial-Robotics/G3Reg

==> sections/tabels/alg_segmentation.tex <==
\begin{algorithm}[t]
	\SetAlgoLined
    \label{alg:plane}
    \caption{Segmentation of LiDAR scan into planes, clusters and lines (PCL)}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{Point cloud $\mathtt{P}$}
    \Output{Low-level semantic segments $\mathtt{PCL}$ and voxel map $\mathtt{V}$}  
    
	\SetKwFunction{mvground}{$\mathtt{RemoveGround}$}
    \SetKwFunction{voxelization}{$\mathtt{Voxelization}$}
    \SetKwFunction{vparse}{$\mathtt{parse}$}
    \SetKwFunction{clustering}{$\mathtt{ObjectClustering}$}
    \SetKwFunction{ransac}{$\mathtt{LineFittingByRANSAC}$}
    \SetKwFunction{relabel}{$\mathtt{ReLabel}$}
	\SetKwFunction{return}{$\mathtt{return}$}

    \SetKwFunction{segmentation}{$\mathtt{PCLSegmentation}$}
    \SetKwProg{Fn}{Function}{}{}
	\Fn{\segmentation{$\mathtt{P}$}}{
        $\mathtt{nonGround} \leftarrow$ \mvground{$\mathtt{P}$};\\
        $V \leftarrow$ \voxelization{$\mathtt{nonGround}$};\\
        \For{$\mathtt{each~voxel~v~in~}$$\mathtt{V}$}{
            $\mathtt{\lambda_k},\mathtt{vec_k}\leftarrow$\vparse{$\mathtt{v}$};\\
            \lIf{$\lambda_2/\lambda_1>20$}{$\mathtt{v.label}\leftarrow\mathtt{plane}$}
        }
        \tcp{Plane merging by region growing}
        $\mathtt{Planes}\leftarrow\emptyset$;\\
        \For{$\mathtt{each~voxel~v~in~}$$\mathtt{V}$}{
            \lIf{$\mathtt{v.label}\neq\mathtt{plane}$}{$\mathtt{continue}$}
            \lIf{$\neg\mathtt{v.init}$}{$\mathtt{plane}\longleftrightarrow\mathtt{v}$}
            \For{$\mathtt{nv~in~}$$\mathtt{v.neighbors}$}{
                \lIf{$\mathtt{nv.label}\neq\mathtt{plane}$}{$\mathtt{continue}$}
                \tcp{Distance, normal and adjacency conditions}
                \eIf{$\mathtt{nv.init~and~DNA(plane, nv.plane)}$}{
                    $\mathtt{plane.merge(nv.plane)}$
                }{
                    \lIf{$\mathtt{\neg nv.init~and~DNA(plane, nv)}$}{
                        $\mathtt{plane.merge(nv)}$
                    }
        		}
            }
            $\mathtt{Planes}\leftarrow\mathtt{plane}$
        }
        $\mathtt{P}\leftarrow \mathtt{P}\setminus \mathtt{planar~points}$;\\
        $\mathtt{Clusters}\leftarrow$\clustering{$\mathtt{P}$};\\
        $\mathtt{Lines}\leftarrow$\ransac{$\mathtt{Clusters}$};\\
        $\mathtt{V}\leftarrow$\relabel{$\mathtt{Planes},\mathtt{Clusters},\mathtt{Lines}$};\\
		\return{$\mathtt{PCL},\mathtt{V}$};
	}
	\textbf{End Function}

    \SetKwFunction{eigensolver}{$\mathtt{eigensolver}$}
    \SetKwProg{Fn}{Function}{}{}
	\Fn{\vparse{$\mathtt{v}$}}{
        $\mathbf{p}_{1:N}\leftarrow\mathtt{v.cloud}$;\\
        $\overline{\mathbf{p}}=\frac{1}{N} \sum_{i=1}^N \mathbf{p}_i$;\\
        $\mathbf{\Sigma}=\frac{1}{N}\left(\mathbf{p}_i-\overline{\mathbf{p}}\right)\left(\mathbf{p}_i-\overline{\mathbf{p}}\right)^{\intercal}$;\\
        \tcp{In the ascending order}
        $\mathtt{\lambda_k},\mathtt{vec_k}\leftarrow$\eigensolver{$\mathtt{\Sigma}$};\\ 
		\return{$\mathtt{\lambda_k},\mathtt{vec_k}$};
	}
	\textbf{End Function}
\end{algorithm}
